Context Attentive Document Ranking and Query Suggestion

We present a context-aware neural ranking model to exploit users' on-task search activities and enhance retrieval performance. In particular, a two-level hierarchical recurrent neural network is introduced to learn search context representation of individual queries, search tasks, and corresponding dependency structure by jointly optimizing two companion retrieval tasks: document ranking and query suggestion. To identify the variable dependency structure between search context and users' ongoing search activities, attention at both levels of recurrent states are introduced. Extensive experiment comparisons against a rich set of baseline methods and an in-depth ablation analysis confirm the value of our proposed approach for modeling search context buried in search tasks.

==> tables/table1.tex <==
\begin{table*}[t]
% \renewcommand{\arraystretch}{1.2}
\centering
% \vspace{-3mm}
\caption{Query suggestions from CARS given all previous queries and their corresponding clicks in a search task.}
\vspace{-2mm}
\begin{tabular}{l|l|l}
\hline
Previous queries from on-going search task & Next query submitted by the user & Query suggested by CARS \\ \hline \hline
\parbox[c]{8cm}{``quotes about june'', ``moon and june quotes''} & \parbox[c]{4.5cm}{quotes about the month of june} & \parbox[c]{4cm}{quotes on love} \\ 
\hline
\parbox[c]{8cm}{``olympus digital'', ``olympus digital mpt player''} & \parbox[c]{4.5cm}{olympus digital m robe 500 drivers} & \parbox[c]{4cm}{olympus stylus 720 sw} \\ 
\hline
% \parbox[c]{8cm}{samsung usa, samsung usa, cell phone reviews} & \parbox[c]{4.5cm}{cell phone reviews} & \parbox[c]{4cm}{samsung cell phone reviews} \\ 
% \hline
\parbox[c][0.8cm]{8cm}{``government grants'', ``government grants for individuals'', ``grants for individuals'', ``personal grants''} & \parbox[c]{4.5cm}{government grants} & \parbox[c]{4cm}{government grants for teachers} \\ 
\hline
\parbox[c][0.8cm]{8cm}{``pathologist and liver cancer'', ``pathologist and liver cancer'', ``hepatitis c and percentage for liver cancer''} & \parbox[c]{4.5cm}{staff infection} & \parbox[c]{4cm}{liver cancer and chemotherapy} 
\\ 
\hline
% \parbox[c][0.8cm]{8cm}{journal of blacks in higher education, grades equivalent to get in to colleges} & \parbox[c]{4.5cm}{grade point average to get in to colleges} & \parbox[c]{4cm}{university of south carolina} 
% \\ 
% \hline
% \parbox[c][0.8cm]{8cm}{graduate degrees theology, southwestern baptist school theology} & \parbox[c]{4.5cm}{mid america seminary} & \parbox[c]{4cm}{theological seminary of america} 
% \\ 
% \hline
\end{tabular}
\label{example:query_suggestion}
\vspace{-1mm}
\end{table*}
